Diffusion Models for Medical Anomaly Detection

In medical applications, weakly supervised anomaly detection methods are of great interest, as only image-level annotations are required for training. Current anomaly detection methods mainly rely on generative adversarial networks or autoencoder models. Those models are often complicated to train or have difficulties to preserve fine details in the image. We present a novel weakly supervised anomaly detection method based on denoising diffusion implicit models. We combine the deterministic iterative noising and denoising scheme with classifier guidance for image-to-image translation between diseased and healthy subjects. Our method generates very detailed anomaly maps without the need for a complex training procedure. We evaluate our method on the BRATS2020 dataset for brain tumor detection and the CheXpert dataset for detecting pleural effusions.

==> brats/auroc.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.75,0.75}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.09)}, anchor=south, draw=white!80!black},
tick align=outside,
tick pos=left,
title={\large \textbf{AUROC}},
x grid style={white!69.0196078431373!black},
xlabel={gradient scale},
xmin=-32.25, xmax=787.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={avg AUROC},
ymin=0.910819466429275, ymax=0.990545201872774,
ytick style={color=black},
ytick={0.91,0.92,0.93,0.94,0.95,0.96,0.97,0.98,0.99,1},
yticklabels={0.91,0.92,0.93,0.94,0.95,0.96,0.97,0.98,0.99,1.00}
]
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
table {%
5 0.980395209479452
10 0.984832099477862
20 0.986027962977908
50 0.986921304807161
100 0.986654321033975
250 0.985492409084434
350 0.984593787390702
500 0.983212486454774
750 0.981348523835677
};
\addlegendentry{L=500}
\addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
table {%
5 0.9341085382295
10 0.951451561706018
20 0.966907618542192
50 0.979228815273021
100 0.982699119742456
250 0.984363445761624
500 0.983443053772777
750 0.983081903789456
};
\addlegendentry{L=250}
\addplot [semithick, black, mark=*, mark size=3, mark options={solid}]
table {%
5 0.963188313854861
10 0.95424934722076
20 0.944176530285981
50 0.929673087283602
100 0.919575126887924
250 0.914443363494889
500 0.91721953508827
750 0.922768287915514
};
\addlegendentry{L=750}
\addplot [semithick, green!50!black, dashed]
table {%
5 0.965
10 0.965
20 0.965
50 0.965
100 0.965
250 0.965
350 0.965
500 0.965
750 0.965
};
\addlegendentry{FP-GAN}
\addplot [semithick, color0, dashed]
table {%
5 0.94
10 0.94
20 0.94
50 0.94
100 0.94
250 0.94
350 0.94
500 0.94
750 0.94
};
\addlegendentry{VAE}
\end{axis}

\end{tikzpicture}


==> brats/prauc.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.75,0.75}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.91,0.5)}, anchor=east, draw=white!80!black},
tick align=outside,
tick pos=left,
title={PR AUC},
x grid style={white!69.0196078431373!black},
xlabel={gradient scale},
xmin=-32.25, xmax=787.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={avg PR AUC},
ymin=0.22047845855589, ymax=0.807691501973529,
ytick style={color=black},
ytick={0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
yticklabels={0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9}
]
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
table {%
5 0.738206404761473
10 0.764792270185239
20 0.770424132413571
50 0.762614582419397
100 0.739647048615249
250 0.689095204067286
350 0.668963649510361
500 0.637391742704233
750 0.608792947615846
};
\addlegendentry{L=500}
\addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
table {%
5 0.404633303012021
10 0.546847602344776
20 0.665251011215209
50 0.746100119058901
100 0.768650718681255
250 0.777077960966204
500 0.766154491931804
750 0.758558202123133
};
\addlegendentry{L=250}
\addplot [semithick, black, mark=*, mark size=3, mark options={solid}]
table {%
5 0.395758932073301
10 0.332319689175225
20 0.283519406614307
50 0.247169960529419
100 0.248679326745228
250 0.280616513935077
500 0.327019218124799
750 0.37351734671986
};
\addlegendentry{L=750}
\addplot [semithick, green!50!black, dashed]
table {%
5 0.781
10 0.781
20 0.781
50 0.781
100 0.781
250 0.781
350 0.781
500 0.781
750 0.781
};
\addlegendentry{FP-GAN}
\addplot [semithick, color0, dashed]
table {%
5 0.276
10 0.276
20 0.276
50 0.276
100 0.276
250 0.276
350 0.276
500 0.276
750 0.276
};
\addlegendentry{VAE}
\end{axis}

\end{tikzpicture}


==> prauc.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.75,0.75}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.91,0.5)}, anchor=east, draw=white!80!black},
tick align=outside,
tick pos=left,
title={PR AUC},
x grid style={white!69.0196078431373!black},
xlabel={gradient scale},
xmin=-32.25, xmax=787.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={avg PR AUC},
ymin=0.22047845855589, ymax=0.807691501973529,
ytick style={color=black},
ytick={0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
yticklabels={0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9}
]
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
table {%
5 0.738206404761473
10 0.764792270185239
20 0.770424132413571
50 0.762614582419397
100 0.739647048615249
250 0.689095204067286
350 0.668963649510361
500 0.637391742704233
750 0.608792947615846
};
\addlegendentry{L=500}
\addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
table {%
5 0.404633303012021
10 0.546847602344776
20 0.665251011215209
50 0.746100119058901
100 0.768650718681255
250 0.777077960966204
500 0.766154491931804
750 0.758558202123133
};
\addlegendentry{L=250}
\addplot [semithick, black, mark=*, mark size=3, mark options={solid}]
table {%
5 0.395758932073301
10 0.332319689175225
20 0.283519406614307
50 0.247169960529419
100 0.248679326745228
250 0.280616513935077
500 0.327019218124799
750 0.37351734671986
};
\addlegendentry{L=750}
\addplot [semithick, green!50!black, dashed]
table {%
5 0.781
10 0.781
20 0.781
50 0.781
100 0.781
250 0.781
350 0.781
500 0.781
750 0.781
};
\addlegendentry{FP-GAN}
\addplot [semithick, color0, dashed]
table {%
5 0.276
10 0.276
20 0.276
50 0.276
100 0.276
250 0.276
350 0.276
500 0.276
750 0.276
};
\addlegendentry{VAE}
\end{axis}

\end{tikzpicture}

